Out-of-Sample Testing for GANs

We propose a new method to evaluate GANs, namely EvalGAN. EvalGAN relies on a test set to directly measure the reconstruction quality in the original sample space (no auxiliary networks are necessary), and it also computes the (log)likelihood for the reconstructed samples in the test set. Further, EvalGAN is agnostic to the GAN algorithm and the dataset. We decided to test it on three state-of-the-art GANs over the well-known CIFAR-10 and CelebA datasets.

==> loss_function.tex <==

\section{Loss Function}
\label{sec:loss_function}

Considering that $\x_i$ an image from the dataset, we have optimize the mean square error between the real and generated sample.
\iffalse
\begin{align}
\label{eq:MSE}
	MSE(\z,\x_i ) = \frac{1}{N}\sum_{i=1}^N( G(\z)- \x_i)^2
\end{align}
\fi
\begin{align}
\label{eq:MSE}
MSE(\z,\x_i ) = \frac{1}{N}\sum_{w=1}^H \sum_{h=1}^W \sum_{k=1}^3( G(\z)[w,h,k]- \x_i[w,h,k])^2
\end{align}

==> old_section3p2.tex <==

\begin{figure}[ht!]
	\begin{center}
		\centerline{\includegraphics[scale=0.6]{images/fig2.pdf}}
		\caption{Cartoon illustrating on how to measure the probability of GAN generated samples.}
		\label{fig2}
	\end{center}
	\vskip -0.2in
\end{figure}

In this paper, we argue that we should not evaluate the likelihood of test samples, but actually the probability of being able to generate them. For example, if we are generating images and we draw $N$ samples from $p(\z)$ how many times do we see a given image. The best way to understand this argument is using the simple cartoon example depicted in Figure \ref{fig2}. We are mapping bijectively (zero-reconstruction error) a one-dimensional uniform distribution $z$ to a 1D sample $x$. %In this case, the reconstruction error will be zero (ignoring the samples outside the uniform range) as there is a bijective function from $z$ to $x$.
 This GAN mapping would generate many instances like $x_2$ and very few like $x_1$. The probability of each $x$ (in this example) depends on the probability of $z$ and on the curvature of $G(\cdot)$ around it. So, wherever $G(\cdot)$ is fairly flat ($F(\cdot)$ is very steep, hence high density), we should expect to see many samples (e.g. $x_2$) and for the regions where $G(\cdot)$ is steep, the probability of seeing those samples would be significantly reduced (e.g. $x_1$). 
 

 
We argue that the relevant measure for evaluating GANs should be:
\begin{equation}
p(\x_{\text{test}})=\int p(\x_c^*|\z)p(\z)d\z,
\end{equation} 
where $\x_c^*$ is the reconstruction of the test sample $\mathbf{x}_{\text{test}}$ from $\z_c^*$ in \eqref{eqz2}. \footnote{We could also use $\x^*=G(\z^*)$ instead, where $\z^*$ is the solution to \eqref{eqz}, but we show in the experimental section that those sample would not be generated when sampling from $p(\z)$. The probability of $p(\x^*)$ would be zero for all practical purposes.} If we set $p(\x_c^*|\z)$ to be a delta function centered at $\z^*_c$ we are left with the likelihood, which is not meaningful, because we cannot capture the curvature of $G(\cdot)$. But given that $G(\cdot)$ is a continuous function and assuming we can allow for some small error, we can readily approximate the probability of seeing each test sample as follows:
\begin{equation}
p(\x_{\text{test}})=\color{red}\int_{\small{d(\x^*_c,G(\z))<T}}p(\z)d\z \color{black} \approx \frac{1}{N}\sum_i \mathbb{I}_{[d(\x^*_c,G(\z_i))<T]}
\end{equation} 
where $T$ is a threshold to ensure that $G(\z_i)$ is close enough to $\x_c^*$, $\z_i$, $i=1,\ldots, N$ are iid samples from $p(\z)$, and $\mathbb{I}_{[d(\x^*_c,G(\z_i))<T]}$ is an indicator function that it is one if the condition holds and zero otherwise. We can set $T$ to be significantly smaller than $d(\x_{\text{test}},\x_c^*)$, which is the error of the best reconstruction of the test sample. Of course for typical GANs, in which the dimension of $\z$ is the hundreds, that approximation is impractical at best. We now present three approximations that can be easily computed. We advocate for the last one, as it is the most computational efficient and accurate of the three.

\paragraph{Isotropic samples.} As we have computed $\z^*_c$ to find $\x_c^*$, we can also approximate this probability as follows:
\begin{equation}\label{L2}
p(\x_{\text{test}})\propto \bar{\sigma}_\epsilon^{\dim(\z)},
\end{equation}
where
\begin{equation}\label{sigmamax}
\bar{\sigma}_\epsilon=\arg\max_{\sigma_\epsilon}\left(\frac{1}{N}\sum_{i=1}^N d(\x_c^*,\x_i^*)\right)\leq T,
\end{equation}
$\x_i^*=G(\z_c^*+\epsilon_i)$, and $\epsilon_i\sim\mathcal{N}(0,\sigma_\epsilon^2\mathbf{I})$. \noteP{We note that, by construction, all $\z_c^*$ have the same probability for all the test samples}, \noteP{and we assume that $\bar{\sigma}_\epsilon$ is small so $p(\z)$ is uniform in a $\bar{\sigma}$-ball around $\z_c^*$, and hence its volume yields \eqref{L2}.} This last condition can be controlled by setting a small enough threshold. 

%Where $T$ is a threshold that ensures that the images generated by adding $\epsilon_i$ are indistinguishable from $\x_c^*$. In this case the likelihood of $\x_c^*$ is given by:

If the curvature of $G(\cdot)$ changes considerably in different dimensions of $\z$ the previous measure benefits those samples that are in a more isotropic region of $G(\cdot)$, because it underestimates the probability of those sample in which $G(\cdot)$ changes significantly in different direction.  

\paragraph{Non-isotropic samples.}  We can adapt the previous measure to account for differences in the curvature of $G(\cdot)$, by computing:
\begin{equation}\label{L3}
p(\x_{\text{test}})\propto N_c^*/N,
\end{equation}
where
\begin{equation}
N_c^*=\sum_{i} \mathbb{I}_{[d(\x^*_c,\x_i^*)<T]},
%\left| \left\{ i |  d(\x_c^*,G(\z_i))\leq T \right\}\right|. 
\end{equation}
and $N_c^*$ counts how many $\x_i^*$ samples  are sufficiently close to $\x_c^*$, when $\sigma_\epsilon$ is small and fixed.

Selecting a good $\sigma_\epsilon$ to ensure that $N_c^*$ is nonzero for a given $N$ and for all the test samples can be hard (and require a very large $N$), if the probability of appearing for all the test samples vary substantially.

\paragraph{Proposed measure.} Finally, by combining the previous two approximations we get:
\begin{equation}\label{L4}
p(\x_{\text{test}})\propto \frac{N_c^*}{N}\bar{\sigma}_\epsilon^{\dim(\z)}.
\end{equation}
This approximation becomes more accurate as we increase $\bar{\sigma}_\epsilon^{\dim(\z)}$, because we are able to capture all the directions in $\z$-space in which the samples $\x_i^*$ are close enough to $\x_c^*$.

For simplicity, for every test sample, we compute this approximation cheaply by fixing $N$ to 1000 and by setting $\bar{\sigma}_\epsilon$ to be the largest value found for which $N_c^*$ is greater than 100. This procedure still favor samples for which the curvature of $G(\cdot)$ is more isotropic, but it mitigates some of the errors produced by the first approximation, while being similarly expensive to compute. By increasing $N$ this problem can be further mitigated. \noteP{Finally, we remark that the proportionality constant in both \eqref{L2},\eqref{L3}, and \eqref{L4} is independent of $\x_{\text{test}}$, and thus the EvalGAN metric can be used for comparing how much probable are certain test samples compared to others.}
%The previous EvalGAN quality step tells us very little about the probability of generating that sample. Because the relation between how good an image can be reconstructed does not need to correlate on how likely we are too see that image when we randomly sample from $p(\z)$. 



%First, when $\z^*$ comes from unconstrained optimization problem in \eqref{eqz}, those samples will never be generated randomly, because the obtained $\z^*$ are either imposible (outside the uniform distribution range) or extremely unlikely (norms too large for Gaussians). Second, if we focus on the solutions to the constrained optimization in \eqref{eqz2}, the likelihood of generating any $\z_c^*$ is exactly the same, because we are either inside the uniform hypercube or we lie on the hypersphere defined by the constraint for the Gaussian case. Third, the likelihood of $\z^*$ or $\z^*_c$ only partly explains the likelihood of the generated samples, because when we generate samples from any GAN, we see that some samples are generate significantly more frequently than others.






%The $\z^*_c$ all have the same likelihood and we need to evaluate the curvature of $G(\cdot)$ around $\z^*_c$ to compute the likelihood for each generated sample. It is important to remark that the methods explained in this subsection are applicable for any $\z$ not only for the $\z^*_c$, they can also be applied to any sample generated by any GAN. For any given $\bar{\z}$ and $\bar{\x}=G(\bar{\z})$ 

%\paragraph{Hessian method.} Given $\z_c^*$ we can construct the following unnormalized density model
%\begin{equation}
%q_u(\z)=\exp\left(-d(G(\z_c^*),G(\z))-\lambda||\z||^2\right)
%\end{equation}
%where $\lambda$ is the Lagrange multiplier for the constraint in \eqref{eqz2}. We can now compute a Laplace approximation around $\z=\z^*_c$ and approximate the likelihood for $\x^*_c$ by:
%\begin{equation}\label{L1}
%L(\x^*_c)\propto \sqrt{|\mathbf{H}_c^*|}, \text{{\color{red} Esta ecuacion puede estar mal}}
%\end{equation}
%where $\mathbf{H}_c^*$ is the Hessian of $q_u(\z_c^*)$. \noteP{We note that the proportionality constant is independent of the image $\x^*_c$.?} 
